kmclib: Automated Inference and Verification of Session Types

Theories and tools based on multiparty session types offer correctness guarantees for concurrent programs that communicate using message-passing. These guarantees usually come at the cost of an intrinsically top-down approach, which requires the communication behaviour of the entire program to be specified as a global type. This paper introduces kmclib: an OCaml library that supports the development of correct message-passing programs without having to write any types. The library utilises the meta-programming facilities of OCaml to automatically infer the session types of concurrent programs and verify their compatibility (k-MC). Well-typed programs, written with kmclib, do not lead to communication errors and cannot get stuck.

==> kmc.tex <==
\subsection{Verifying $k$-Multiparty Compatibility}\label{subsec:kmc}
%
The notion of $k$-multiparty compatibility was introduced
in~\cite{LangeY19} as a sound procedure to determine the safety of a
sub-class of CFSMs corresponding to session types.
%
The definition of \kmc consists of two components: $k$-exhaustivity
and $k$-safety that rely on $k$-bounded executions, i.e., executions
where each channel contains at most $k$ messages.
%
%
A system of CFSMs is $k$-exhaustive if for all its $k$-bounded
execution, all send actions are enabled within this bounds.
%
A system is $k$-safe if for all its $k$-bounded executions,
no machine gets permanently stuck in a receiving state and all sent
messages are eventually received.

We say that a system is \kmc if there is $k \in \mathbb{N}$ such that
it is both $k$-exhaustive and $k$-safe.
%

If a system if \kmc, then it is safe in the sense that no machine gets
permanently stuck in a receiving state and all sent messages are
eventually received.
%
Additionally, $k$-exhaustivity guarantees that each role locally
behaves equivalently under any bound greater than or equal to
$k$. \JLnote{Link back to something about transport}
%
If a system is $k$-exhaustive but not $k$-safe, then it contains
executions that either violate progress or eventual reception.

The tool from~\cite{LangeY19} performs a bounded verification to
discover the least $k$ for which a system is $k$-MC (up-to a specified
bound).
%
We have adapted it in~\cite{KMC} so that it returns counter example of
traces that violate $k$-safety. \JLnote{Link back to ocaml side}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

